Estimation with Norm Regularization

Analysis of non-asymptotic estimation error and structured statistical recovery based on norm regularized regression, such as Lasso, needs to consider four aspects: the norm, the loss function, the design matrix, and the noise model. This paper presents generalizations of such estimation error analysis on all four aspects compared to the existing literature. We characterize the restricted error set where the estimation error vector lies, establish relations between error sets for the constrained and regularized problems, and present an estimation error bound applicable to any norm. Precise characterizations of the bound is presented for isotropic as well as anisotropic subGaussian design matrices, subGaussian noise models, and convex loss functions, including least squares and generalized linear models. Generic chaining and associated results play an important role in the analysis. A key result from the analysis is that the sample complexity of all such estimators depends on the Gaussian width of a spherical cap corresponding to the restricted error set. Further, once the number of samples $n$ crosses the required sample complexity, the estimation error decreases as $\frac{c}{\sqrt{n}}$, where $c$ depends on the Gaussian width of the unit norm ball.

==> main-gauss-re.tex <==
Here we focus on the case of Gaussian design matrices $X \in \R^{n \times p}$,
and consider three settings: (i) independent-isotropic, where the entries are elementwise independent, (ii) independent-anisotropic, where rows $X_i$ are independent but each row has a covariance $E[X_i X_i^T] = \Sigma \in \R^{p \times p}$, and (iii) dependent-isotropic, where the rows are isotropic but the columns $X_j$ are correlated with $E[X_j X_j^T] = \Gamma \in \R^{n \times n}$. For convenience, we assume $E[x_{ij}^2] = 1$, noting that the analysis easily extends to the general case of $E[x_{ij}^2] = \sigma^2$.



%\subsubsection{Independent Isotropic Gaussian (IIG) Designs}
%\label{sssec:iig}
{\bf Independent Isotropic Gaussian (IIG) Designs:}
The IIG setting has been extensively studied in the literature~\cite{buva11,nrwy12}. As discussed in the recent work on atomic norms~\cite{crpw12}, one can use Gordon's inequality~\cite{gord88,ledo13} to get RE conditions for the IIG setting. Our goal here is two-fold: first, we present the RE conditions obtained using our simple proof technique, and show that it is equivalent, up to constants, the RE condition obtained using Gordon's inequality, an arguably heavy-duty technique only applicable to the IIG setting; and second, we go over some facets of how we present the results, which will apply to all subsequent RE-style results as well as give a way to plug-in $\kappa$ in the estimation error bound in~\myref{eq:recover}.
\begin{theo}
Let the design matrix $X \in \R^{n \times p}$ be elementwise independent and normal, i.e., $x_{ij} \sim N(0,1)$. Then, for any $A \subseteq S^{p-1}$, any $n \geq 2$, and any $\tau > 0$, with probability at least $(1-\eta_1\exp(-\eta_2 \tau^2))$, we have
\beq
\inf_{u \in A} \| X u \|_2  \geq \frac{1}{2}\sqrt{n} - \eta_0 w(A) - \tau~,
\eeq
$\eta_0,\eta_1, \eta_2 > 0$ are absolute constants.
\label{thm:re-iig}
\end{theo}
As a result, the sample complexity $n_A = O(w^2(A))$.
We consider the equivalent result one could obtain by directly using Gordon's inequality~\cite{gord88,ledo13}:
\begin{theo}[Gordon's inequality~\cite{gord88}]
Let the design matrix $X$ be elementwise independent and normal, i.e., $x_{ij} \sim N(0,1)$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-2\exp(-\tau^2/2))$, we have
\beq
\inf_{u \in A} \| X u \|_2  \geq \gamma_n - w(A) - \tau~,
\eeq
where $\gamma_n = E[\| g \|_2] > \frac{n}{\sqrt{n+1}}$ is the expected length of a Gaussian random vector in $\R^n$.
\label{thm:re-iig2}
\end{theo}
Interestingly, the results are equivalent up to constants. However, unlike Gordon's inequality, our proof technique generalizes to other design matrices, including sub-Gaussian designs.

We emphasize three additional aspects in the context of the above analysis, which will continue to hold for all the subsequent results but will not be discussed explicitly. First, to get a form of the result which can be used as $\kappa$ and plugged in to the estimation error bound \myref{eq:recover}, one can simply choose $\tau = \frac{1}{2} (\frac{1}{2} \sqrt{n} - \eta_0 w(A))$ so as to get
\vspace*{-2mm}
\beq
\inf_{u \in A} \| X u \|_2 \geq \frac{1}{4} \sqrt{n} - \frac{\eta_0}{2} w(A)~,
\eeq
with high probability.
Second, the result does not depend on the size of $u$, i.e., $\|u\|_2$. For the above analysis, $u \in A \subseteq C_r \cap S^{p-1}$ so that $\| u \|_2 = 1$. However, one can consider the cone $C_r$ to be intersecting with a sphere $\rho S^{p-1}$ of a different radius $\rho$, to give $A_{\rho} = C_r \cap \rho S^{p-1}$ so that $u \in A_{\rho}$ has $\| u \|_2 = \rho$. For simplicity, let $A = A_1$, i.e., corresponding to $\rho = 1$. Then, a straightforward extension yields
%\beq
$\inf_{u \in A_{\rho}} \| X u \|_2 \geq (\frac{1}{2} \sqrt{n} - \eta_0 w(A) - \tau) \| u \|_2$,
%\eeq
with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$,
since $\| X u \|_2 = \| X \frac{u}{\|u\|_2} \|_2 \| u \|_2$ and $w(A_{\|u\|_2}) =  \| u \|_2 w(A)$~\cite{crpw12}. %Such a scale independence is sufficient for the error bound analysis in Section~\ref{sec:error}. 
Finally, note that the leading constant $\frac{1}{2}$ was a consequence of our choice of $\epsilon = \frac{1}{4}$ for the $\epsilon$-net covering of $A$ in the proof. One can get other constants, less than 1, with different choices of $\epsilon$, and the constants $\eta_0,\eta_1,\eta_2$ will change based on this choice.


%\subsubsection{Independent Anisotropic Gaussian (IAG) Designs}
%\label{sssec:iag}

{\bf Independent Anisotropic Gaussian (IAG) Designs:}
We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled from an anisotropic Gaussian distribution, i.e., $X_i \sim N(0, \Sigma_{p \times p})$ where $X_i \in \R^p$. The setting has been considered in the literature~\cite{rawy10} for the special case of $L_1$ norms, and results have been established using Gaussian comparison techniques~\cite{ledo13}. We show that equivalent results can be obtained by our simple technique, which does not rely on Gaussian comparisons~\cite{ledo13,nrwy12}.
\begin{theo}
Let the design matrix $X$ be row wise independent and each row $X_i \sim N(0,\Sigma_{p \times p})$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $1 - \eta_1 \exp(-\eta_2 \tau^2)$, we have
\beq
\inf_{u \in A} \| X u \|_2 \geq \frac{1}{2} \sqrt{\nu}\sqrt{n} - \eta_0 \sqrt{\Lambda_{\max}(\Sigma)}~ w(A) - \tau~,
\eeq
where $\sqrt{\nu} = \inf_{u \in A} \| \Sigma^{1/2} u \|_2$, $\Lambda_{\max}(\Sigma)$ denotes the largest eigenvalue of $\Sigma$ and $\eta_0,\eta_1, \eta_2 > 0$ are constants.
\label{thm:re-iag}
\end{theo}
As a result, the sample complexity $n_A = O(\lambda_{\max}(\Sigma) w^2(A)/\nu)$.
A comparison with the results of~\cite{rawy10} is instructive. The leading term $\sqrt{\nu}$ appears in both results---the result in~\cite{rawy10} is for any $u$ and has a $\| \Sigma^{1/2} u \|_2$ term, whereas we have simply considered $\inf_{u \in A}$ on both sides. The second term in~\cite{rawy10} depends on the largest entry in the diagonal of $\Sigma$, $\sqrt{\log p}$, and $\| u \|_1$. These terms are a consequence of the special case analysis for $L_1$ norm. In contrast, we consider the general case and simply get the scaled Gaussian width term $\sqrt{\Lambda_{\max}}(\Sigma)w(A)$.

%The constant in the Gaussian width term above relies on the largest eigenvalue of $\Sigma^{1/2}$ whereas in~\cite{rawy10} the constant depends on the largest entry in the diagonal and also the $L_1$ norm of the error vector $u$.

%which is sharper and is the advantage of using the Gaussian comparison technique~\cite{ledo13}.

%\subsubsection{Dependent Isotropic Gaussian (DIG) Designs}
%\label{sssec:dig}

{\bf Dependent Isotropic Gaussian (DIG) Designs:}
We now consider a setting where the rows of the design matrix $\tilde{X}$ are isotropic Gaussians, but the columns $\tilde{X}_j$ are correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma \in \R^{n \times n}$.
Interestingly, correlation structure over the columns make the samples dependent, a scenario which has not yet been widely studied in the literature~\cite{zhou14,newa11}. We show that our simple technique continues to work in this scenario and gives a rather intuitive result.
\begin{theo}
Let $\tilde{X} \in \R^{n \times p}$ be a matrix whose rows $\tilde{X}_i$ are isotropic Gaussian random vectors in $\R^p$ and the columns $\tilde{X}_j$ are correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma$. Then, for any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1 - \eta_1 \exp (-\eta_2 \tau^2)$, we have
\beq
\inf_{u \in A}~ \| \tilde{X} u \|_2 \geq \frac{3}{4}\sqrt{\tr(\Gamma)} - \sqrt{\Lambda_{\max}(\Gamma)}~ \left( \eta_0 w(A) + \frac{5}{2} \right) - \tau
\eeq
where $\eta_0,\eta_1, \eta_2 > 0$ are constants.
\label{thm:corrG}
\end{theo}
Note that with the assumption that $E[x_{ij}^2] = 1$, $\Gamma$ will be a correlation matrix implying $\tr(\Gamma) = n$, and making the sample size dependence explicit. Intuitively, due to sample correlations, $n$ samples are effectively equivalent to $\frac{\tr(\Gamma)}{\Lambda_{\max}(\Gamma)}=\frac{n}{\Lambda_{\max}(\Gamma)}$ samples. For the special case of $\Gamma = \mathbb{I}_{n \times n}$, $\tr(\Gamma) = n$, $\Lambda_{\max}(\Gamma)$ = 1, and we recover the result for IIG designs.











%In this section, we focus on the case of Gaussian design matrices $X \in \R^{n \times p}$,
%and consider three settings: (i) independent-isotropic, where the entries are elementwise independent, (ii) independent-anisotropic, where %individual rows $X_i$ are independent but each row has a covariance $E[X_i X_i^T] = \Sigma \in \R^{p \times p}$, and (iii) %dependent-isotropic, where the columns $X_j$ are correlated with $E[X_j X_j^T] = \Gamma \in \R^{n \times n}$ and the rows are isotropic. For %convenience, we assume $E[x_{ij}^2] = 1$, noting that the analysis easily extends to the general case of $E[x_{ij}^2] = \sigma^2$.



%\subsubsection{Independent Isotropic Gaussian (IIG) Designs}
%\label{sssec:iig}
%{\bf Independent Isotropic Gaussian (IIG) Designs:}
%The IIG setting has been extensively studied in the literature~\cite{buva11,nrwy12}. As discussed in the recent work on atomic %norms~\cite{crpw12}, one can use Gordon's inequality~\cite{gord85,gord88,ledo13} to get RE conditions for the IIG setting. Our goal in %this section is two-fold: first, we present the RE conditions obtained using our simple proof technique, and show that it is equivalent, up %to constants, the RE condition obtained using Gordon's inequality, an arguably heavy-duty technique only applicable to the IIG setting; and %second, we go over some facets of how we present the results, which will apply to all subsequent RE-style results as well as give a way to %plug-in $\kappa$ in the estimation error bound in~\myref{eq:recover}.
%\begin{theo}
%Let the design matrix $X \in \R^{n \times p}$ be elementwise independent and normal, i.e., $x_{ij} \sim N(0,1)$. Then, for any $A \subseteq %S^{p-1}$, any $n \geq 2$, and any $\tau > 0$, with probability at least $(1-\eta_1\exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2  \geq \frac{1}{2}\sqrt{n} - \eta_0 w(A_r) - \tau~,
%\eeq
%$\eta_0,\eta_1, \eta_2 > 0$ are absolute constants.
%\label{thm:re-iig}
%\end{theo}
%We consider the equivalent result one could obtain by directly using Gordon's inequality~\cite{gord85,gord88,ledo13}:
%\begin{theo}
%Let the design matrix $X$ be elementwise independent and normal, i.e., $x_{ij} \sim N(0,1)$. Then, for any $A \subseteq S^{p-1}$ and any %$\tau > 0$, with probability at least $(1-2\exp(-\tau^2/2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2  \geq \gamma_n - w(A_r) - \tau~,
%\eeq
%where $\gamma_n = E[\| h \|_2] > \frac{n}{\sqrt{n+1}}$ is the expected length of a Gaussian random vector in $\R^n$.
%\label{thm:re-iig2}
%\end{theo}
%Interestingly, the results are equivalent, up to constants. In fact, our technique provides an alternative proof to Gordon's inequality %using a covering argument, and not using Gaussian comparison techniques~\cite{dudl67,nrwy12,ledo13}.

%We emphasize three additional aspects in the context of the above analysis, which will continue to hold for all the subsequent results but %will not be discussed explicitly. First, to get a form of the result which can be used as $\kappa$ and plugged in to the estimation error %bound \myref{eq:recover}, one can simply choose $\tau = \frac{1}{2} (\frac{1}{2} \sqrt{n} - \eta_0 w(A))$ so as to get
%\vspace*{-2mm}
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \frac{1}{4} \sqrt{n} - \frac{\eta_0}{2} w(A)~,
%\eeq
%with probability at least $1 - c_1 \exp( - c_2 n)$ for suitable constants $c_1, c_2 >0$. Second, the result does not depend on the fact that %$u \in A \subseteq C \cap S^{p-1}$ so that $\| u \|_2 = 1$. For example, one can consider the cone $C$ to be intersecting with a sphere %$\rho S^{p-1}$ of a different radius $\rho$, to give $A_{\rho} = C \cap \rho S^{p-1}$ so that $u \in A_{\rho}$ has $\| u \|_2 = \rho$. For %simplicity, let $A = A_1$, i.e., corresponding to $\rho = 1$. Then, a straightforward extension yields
%%\beq
%$\inf_{u \in A_{\rho}} \| X u \|_2 \geq (\frac{1}{2} \sqrt{n} - \eta_0 w(A) - \tau) \| u \|_2$,
%\eeq
%with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$,
%since $\| X u \|_2 = \| X \frac{u}{\|u\|_2} \|_2 \| u \|_2$ and $w(A_{\|u\|_2}) =  \| u \|_2 w(A_1)$~\cite{crpw12}. Such a scale %independence is in fact necessary for the error bound analysis in Section~\ref{sec:error}. Finally, note that the leading constant %$\frac{1}{2}$ was a consequence of our choice of $\epsilon = \frac{1}{4}$ for the $\epsilon$-net covering of $A$ in the proof. One can get %other constants, less than 1, with different choices of $\epsilon$, and the constants $\eta_0,\eta_1,\eta_2$ will change based on this c %hoice.


%\subsubsection{Independent Anisotropic Gaussian (IAG) Designs}
%\label{sssec:iag}

%{\bf Independent Anisotropic Gaussian (IAG) Designs:}
%We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled from an anisotropic Gaussian %distribution, i.e., $X_i \sim N(0, \Sigma)$ where $X_i \in \R^p$. The setting has been considered in the literature~\cite{rawy10} for %the special case of $L_1$ norms, and sharp results have been established using Gaussian comparison techniques~\cite{ledo13}. We show that %equivalent results can be obtained by our simple technique, which does not rely on Gaussian comparisons~\cite{ledo13,nrwy12}.
%\begin{theo}
%Let the design matrix $X$ be row wise independent and each row $X_i \sim N(0,\Sigma)$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > %0$, with probability at least $1 - \eta_1 \exp(-\eta_2 \tau^2)$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \frac{1}{2} \sqrt{\nu}\sqrt{n} - \eta_0 \sqrt{\Lambda_{\max}(\Sigma)}~ w(A) - \tau~,
%\eeq
%where $\sqrt{\nu} = \inf_{u \in A} \| \Sigma^{1/2} u \|_2$ and $\sqrt{\Lambda_{\max}(\Sigma)}$ denotes the largest eigenvalue of %$\Sigma^{1/2}$.
%\label{thm:re-iag}
%\end{theo}
%A comparison with the results of~\cite{rawy10} is instructive. The leading term $\sqrt{\nu}$ appears in~\cite{rawy10} as %well---where we have taken the $\inf_{u \in A}$, the result in~\cite{rawy10} is for any $u$ with the $\| \Sigma^{1/2} u \|_2$ term. The %constant in the Gaussian width term above relies on the largest eigenvalue of $\Sigma^{1/2}$ whereas in~\cite{rawy10} the constant %depends on the largest entry in the diagonal, which is sharper and is the advantage of using the Gaussian comparison %technique~\cite{ledo13}.

%\subsubsection{Dependent Isotropic Gaussian (DIG) Designs}
%\label{sssec:dig}

%{\bf Dependent Isotropic Gaussian (DIG) Designs:}
%We now consider a setting where the rows of the design matrix $\tilde{X}$ are isotropic Gaussians, but the columns $\tilde{X}_j$ are %correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma \in \R^{n \times n}$.
%Interestingly, correlation structure over the columns make the samples dependent, a scenario which has not yet been widely studied in the %literature~\cite{zhou14,newa11}. We show that our simple technique continues to work in this scenario and gives a rather intuitive result.
%\begin{theo}
%Let $\tilde{X} \in \R^{n \times p}$ be a matrix whose rows $\tilde{X}_i$ are isotropic Gaussian random vectors in $\R^p$ and the columns %$\tilde{X}_j$ are correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma$. Then, for any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with %probability at least $(1 - \eta_1 \exp (-\eta_2 \tau^2)$, we have
%\beq
%\inf_{u \in A}~ \| \tilde{X} u \|_2 \geq \frac{3}{4}\sqrt{\tr(\Gamma)} - \sqrt{\Lambda_{\max}(\Gamma)}~ \left( \eta_0 w(A) + \frac{5}{2} %\right) - \tau
%\eeq
%where $\eta_0,\eta_1, \eta_2 > 0$ are constants.
%\label{thm:corrG}
%\end{theo}
%Note that with the assumption that $E[x_{ij}^2] = 1$, $\Gamma$ will be a correlation matrix implying $\tr(\Gamma) = n$, and making the %sample size dependence explicit. Intuitively, due to sample correlations, $n$ samples are effectively equivalent to %$\frac{\tr(\Gamma)}{\Lambda_{\max}(\Gamma)}=\frac{n}{\Lambda_{\max}(\Gamma)}$ samples.



==> main-relwork.tex <==
I also suggest discussing recent developments that
also extend [1] and use Gordon's lemma extensively: work by Oymak
(http://arxiv.org/abs/1311.0830 is the most recent and most comprehensive)
and work by McCoy and Amelunxen and co-authors (again,
http://arxiv.org/abs/1303.6672 is their most recent and most comprehensive).
For example, Oymak's paper has a strong framework that covers this current
paper, and all you need to do is plug in estimates for the cones (in the form of
Gaussian widths or the "Gaussian squared-distances to the subdifferential cone"
or the "statistical dimension").

==> main-subgauss-re.tex <==
In this section, we focus on the case of sub-Gaussian design matrices $X \in \R^{n \times p}$, and consider
three settings: (i) independent-isotropic, where the rows are independent and isotropic, (ii) independent-anisotropic, where the rows $X_i$ are independent but each row has a covariance $E[X_iX_i^T] =
\Sigma_{p \times p}$, and (iii) dependent-isotropic, where the rows are isotropic and the columns $X_j$ are correlated with $E[X_j X_j^T] = \Gamma_{n \times n}$. For convenience, we assume $E[x_{ij}^2] = 1$ and the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} \leq k$~\cite{vers12}. In recent work, building on \cite{mend14}, \cite{trop14} also considers generalizations of RE conditions to sub-Gaussian designs, although our proof techniques are different.


%In this section, we focus on the setting where the design matrix $X \in \R^{n \times p}$ has sub-Gaussian entries. There is some existing literature on gain conditions with sub-Gaussian entries, primarily focussed on independent rows of isotropic sub-Gaussian vectors for a few specific choices of norms [][]. Further, [] established results on anisotropic sub-Gaussian design matrices for the setting of $L_1$ norm. Similar to our treatment of Gaussian design matrices, we consider three settings, involving independent isotropic designs, independent anisotropic designs, and dependent isotropic designs. Our analysis applies to all norms and the dependency is captured in terms of the Gaussian width of the error cone induced by the norm. Interestingly, although we are dealing with sub-Gaussian designs, the results include the Gaussian width, since we use the Gaussian width to measure size of the error set $A$ and the sub-Gaussian aspect only determines the suitable large deviation bounds.

%\subsubsection{Independent Isotropic Sub-Gaussian Designs}
%\label{sssec:iisg}

{\bf Independent Isotropic Sub-Gaussian Designs:} We start with the setting where the sub-Gaussian design matrix $X \in \R^{n \times p}$ has independent rows $X_i$ and each row is isotropic.
\vspace*{-2mm}
%so that $E[x_{ij}^2] = 1$. Further, we assume that the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\begin{theo}
%Let $X \in \R^{n \times p}$ be a design matrix whose rows $X_i$ are independent isotropic sub-Gaussian random vectors in $R^p$. Then, for %any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \frac{3}{4} \sqrt{n} - \eta_0 w(A) - \sqrt{2} k_0 - \tau~,
%\eeq
%where $k_0,\eta_0,\eta_1,\eta_2 > 0$ are constants which depend on the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$.
%\label{thm:iisg}
%\end{theo}
\begin{theo}
Let $X \in \R^{n \times p}$ be a design matrix whose rows $X_i$ are independent isotropic sub-Gaussian random vectors in $R^p$. Then, for any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-2 \exp(-\eta_1 \tau^2))$, we have
\beq
\inf_{u \in A} \| X u \|_2 \geq \sqrt{n} - \eta_0 w(A) - \tau~,
\eeq
where $\eta_0, \eta_1 > 0$ are constants which depend only on the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$.
\vspace*{-3mm}
\label{thm:iisg2}
\end{theo}
As in the case of Gaussian designs, the sample complexity $n_A = O(w^2(A))$.
%We present an alternative result, using a variant of the covering argument~\cite{vers12}, which leads to mildly
%better constants in the deviation amount, e.g., the $\sqrt{2}k_0$ term disappears, but with worse constants for the probability bound, i.e., %$\eta_2 \propto \frac{1}{k^4}$ in Theorem~\ref{thm:iisg2} as opposed to $\eta_2 \propto \frac{1}{k^2}$ in the above Theorem~\ref{thm:iisg}.
%\begin{theo}
%Let $X \in \R^{n \times p}$ be a design matrix whose rows $X_i$ are independent isotropic sub-Gaussian random vectors in $R^p$. Then, for %any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \sqrt{n} - \eta_0 w(A) - \tau~,
%\eeq
%where $\eta_0,eta_1, \eta_2 > 0$ are constants which depend only the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$.
%\label{thm:iisg2}
%\end{theo}

%\subsubsection{Independent Anisotropic Sub-Gaussian Designs}
%\label{sssec:re-iasg}

{\bf Independent Anisotropic Sub-Gaussian Designs:}
We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled
from an anisotropic sub-Gaussian distribution, i.e., $\vertiii{x_{ij}}_{\psi_2} = k$ and $E[X_i X_i^T] = \Sigma_{p \times p}$.
%
%We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled from an anisotropic sub-Gaussian distribution, i.e., $\vertiii{x_{ij}}_{\psi_2} = k$ and $E[X_i X_i^T] \sim N(0, \Sigma)$ where $X_i \in \R^p$. Further, to maintain the results at the same scale as previous results, we assume $\vertiii{x_{ij}}_2 = 1$ without loss of generality. The setting of anisotropic sub-Gaussian design matrices has been investigated in [] for the special case of $L_1$ norm. In contrast, our analysis applies to any norm regularization with dependency captured by the Gaussian width of the corresponding error set. Further, the analysis can be viewed as an extension of our general proof technique used in earlier sections.
%
%\begin{theo}
%Let the sub-Gaussian design matrix $X$ be row wise independent, and each row has  $E[X_i X_i^T] = \Sigma \in \R^{p \times p}$. Then, for any %$A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \frac{3}{4} \sqrt{\nu} \sqrt{n}  - \eta_0 \sqrt{\Lambda_{\max}(\Sigma)}~w(A) - \sqrt{2\nu} k_0 - \tau~,
%\eeq
%where $\sqrt{\nu} = \inf_{u \in A} \| \Sigma^{1/2} u \|_2$, $\sqrt{\Lambda_{\max}(\Sigma)}$ denotes the largest eigenvalue of %$\Sigma^{1/2}$, and $k_0,\eta_0,\eta_1,\eta_2 > 0$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\label{thm:re-iasg}
%\end{theo}
\vspace*{-2mm}
\begin{theo}
Let the sub-Gaussian design matrix $X$ be row wise independent, and each row has  $E[X_i X_i^T] = \Sigma \in \R^{p \times p}$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-2 \exp(-\eta_1 \tau^2))$, we have
\beq
\inf_{u \in A} \| X u \|_2 \geq \sqrt{\nu} \sqrt{n}  - \eta_0~ \Lambda_{\max}(\Sigma)~w(A) - \tau~,
\eeq
where $\sqrt{\nu} = \inf_{u \in A} \| \Sigma^{1/2} u \|_2$, $\Lambda_{\max}(\Sigma)$ denotes the largest eigenvalue of $\Sigma$, and $\eta_0,\eta_1 > 0$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
\vspace*{-3mm}
\label{thm:re-iasg}
\end{theo}
As a result, the sample complexity $n_A = O(\lambda_{\max}^2(\Sigma) w^2(A)/\nu)$.
Note that~\cite{ruzh13} establish RE conditions for anisotropic sub-Gaussian designs for the special case of $L_1$ norm. In contrast, our results are general and in terms of the Gaussian width $w(A)$.


%\subsubsection{Dependent Isotropic Sub-Gaussian Designs}
%\label{sssec:disg}

{\bf Dependent Isotropic Sub-Gaussian Designs:}
We consider the setting where the sub-Gaussian design matrix $\tilde{X}$ has isotropic sub-Gaussian rows, but the columns $\tilde{X}_j$ are correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma$, implying dependent samples.
%In particular, we assume that $\| \tilde{x}_{ij} \|_{\psi_2} = k$,
%and $E[\tilde{X} \tilde{X}^T] = \Gamma \in \R^{n \times n}$. We show that the gain condition holds for such dependent sub-Gaussian designs:
%\begin{theo}
%Let $\tilde{X} \in \R^{n \times p}$ be a sub-Gaussian design matrix with isotropic rows and correlated columns with $E[\tilde{X}_j %\tilde{X}_j^T] = \Gamma \in \R^{n \times n}$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1- \eta_1 %\exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| \tilde{X} u \|_2 \geq \frac{3}{4} \sqrt{\tr(\Gamma)} -  \sqrt{\Lambda_{\max}(\Gamma)}~(\eta_0 w(A) + \sqrt{2}k_0  - \tau~,
%\eeq
%where $k_0,\eta_0, \eta_1, \eta_2$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\label{thm:corrSubG}
%\end{theo}
\vspace*{-2mm}
\begin{theo}
Let $\tilde{X} \in \R^{n \times p}$ be a sub-Gaussian design matrix with isotropic rows and correlated columns with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma \in \R^{n \times n}$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1- 2 \exp(-\eta_1 \tau^2) )$, we have
\beq
\inf_{u \in A} \| \tilde{X} u \|_2 \geq \sqrt{\tr(\Gamma)} - \eta_0~ \Lambda_{\max}(\Gamma) w(A)  - \tau~,
\eeq
where $\eta_0, \eta_1$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
\label{thm:corrSubG}
\end{theo}



%In this section, we focus on the case of sub-Gaussian design matrices $X \in \R^{n \times p}$, and consider
%three settings: (i) independent-isotropic, where the rows independent and isotropic, (ii) independent-anisotropic, where the rows $X_i$ are %independent but each row has a covariance $E[X_iX_i^T] =
%\Sigma_{\p \times p}$, and (iii) dependent-isotropic, where the rows are isotropic and the columns $X_j$ are correlated with $E[X_j X_j^T] = %\Gamma_{n \times n}$. For convenience, we assume $E[x_{ij}^2] = 1$ and the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$~\cite{vers12}.


%In this section, we focus on the setting where the design matrix $X \in \R^{n \times p}$ has sub-Gaussian entries. There is some existing literature on gain conditions with sub-Gaussian entries, primarily focussed on independent rows of isotropic sub-Gaussian vectors for a few specific choices of norms [][]. Further, [] established results on anisotropic sub-Gaussian design matrices for the setting of $L_1$ norm. Similar to our treatment of Gaussian design matrices, we consider three settings, involving independent isotropic designs, independent anisotropic designs, and dependent isotropic designs. Our analysis applies to all norms and the dependency is captured in terms of the Gaussian width of the error cone induced by the norm. Interestingly, although we are dealing with sub-Gaussian designs, the results include the Gaussian width, since we use the Gaussian width to measure size of the error set $A$ and the sub-Gaussian aspect only determines the suitable large deviation bounds.

%\subsubsection{Independent Isotropic Sub-Gaussian Designs}
%\label{sssec:iisg}

%{\bf Independent Isotropic Sub-Gaussian Designs:} We start with the setting where the sub-Gaussian design matrix $X \in \R^{n \times p}$ has %independent rows $X_i$ and each row is isotropic.
%so that $E[x_{ij}^2] = 1$. Further, we assume that the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\begin{theo}
%Let $X \in \R^{n \times p}$ be a design matrix whose rows $X_i$ are independent isotropic sub-Gaussian random vectors in $R^p$. Then, for any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-\eta_1 \exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \frac{3}{4} \sqrt{n} - \eta_0 w(A) - \sqrt{2} k_0 - \tau~,
%\eeq
%where $k_0,\eta_0,\eta_1,\eta_2 > 0$ are constants which depend on the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$.
%\label{thm:iisg}
%\end{theo}
%We present an alternative result, using a variant of the covering argument~\cite{vers12}, which leads to mildly
%better constants in the deviation amount, e.g., the $\sqrt{2}k_0$ term disappears, but with worse constants for the probability bound, i.e., $\eta_2 \propto \frac{1}{k^4}$ in Theorem~\ref{thm:iisg2} as opposed to $\eta_2 \propto \frac{1}{k^2}$ in the above Theorem~\ref{thm:iisg}.
%\begin{theo}
%Let $X \in \R^{n \times p}$ be a design matrix whose rows $X_i$ are independent isotropic sub-Gaussian random vectors in $R^p$. Then, for %any set $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-2 \exp(-\eta_1 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \sqrt{n} - \eta_0 w(A) - \tau~,
%\eeq
%where $\eta_0, \eta_1 > 0$ are constants which depend only the sub-Gaussian norm $\vertiii{x_{ij}}_{\psi_2} = k$.
%\label{thm:iisg2}
%\end{theo}

%\subsubsection{Independent Anisotropic Sub-Gaussian Designs}
%\label{sssec:re-iasg}

%{\bf Independent Anisotropic Sub-Gaussian Designs:}
%We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled
%from an anisotropic sub-Gaussian distribution, i.e., $\vertiii{x_{ij}}_{\psi_2} = k$ and $E[X_i^T X_i] = \Sigma_{p \times p}$.
%
%We consider a setting where the rows $X_i$ of the design matrix are independent, but each row is sampled from an anisotropic sub-Gaussian distribution, i.e., $\vertiii{x_{ij}}_{\psi_2} = k$ and $E[X_i X_i^T] \sim N(0, \Sigma)$ where $X_i \in \R^p$. Further, to maintain the results at the same scale as previous results, we assume $\vertiii{x_{ij}}_2 = 1$ without loss of generality. The setting of anisotropic sub-Gaussian design matrices has been investigated in [] for the special case of $L_1$ norm. In contrast, our analysis applies to any norm regularization with dependency captured by the Gaussian width of the corresponding error set. Further, the analysis can be viewed as an extension of our general proof technique used in earlier sections.
%
%\begin{theo}
%Let the sub-Gaussian design matrix $X$ be row wise independent, and each row has  $E[X_i X_i^T] = \Sigma \in \R^{p \times p}$. Then, for any %$A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1-2 \exp(-\eta_1 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| X u \|_2 \geq \sqrt{\nu} \sqrt{n}  - \eta_0 \Lambda_{\max}(\Sigma)~w(A) - \tau~,
%\eeq
%where $\sqrt{\nu} = \inf_{u \in A} \| \Sigma^{1/2} u \|_2$, $\sqrt{\Lambda_{\max}(\Sigma)}$ denotes the largest eigenvalue of %$\Sigma^{1/2}$, and $k_0,\eta_0,\eta_1,\eta_2 > 0$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\label{thm:re-iasg}
%\end{theo}



%\subsubsection{Dependent Isotropic Sub-Gaussian Designs}
%\label{sssec:disg}

%{\bf Dependent Isotropic Sub-Gaussian Designs:}
%We consider the setting where the sub-Gaussian design matrix $\tilde{X}$ has isotropic sub-Gaussian rows, but the columns $tilde{X}_j$ are %correlated with $E[\tilde{X}_j \tilde{X}_j^T] = \Gamma$, implying dependent samples.
%In particular, we assume that $\| \tilde{x}_{ij} \|_{\psi_2} = k$,
%and $E[\tilde{X} \tilde{X}^T] = \Gamma \in \R^{n \times n}$. We show that the gain condition holds for such dependent sub-Gaussian designs:
%\begin{theo}
%Let $\tilde{X} \in \R^{n \times p}$ be a sub-Gaussian design matrix with isotropic rows and correlated columns with $E[\tilde{X}_j %\tilde{X}_j^T] = \Gamma \in \R^{n \times n}$. Then, for any $A \subseteq S^{p-1}$ and any $\tau > 0$, with probability at least $(1- \eta_1 \exp(-\eta_2 \tau^2))$, we have
%\beq
%\inf_{u \in A} \| \tilde{X} u \|_2 \geq \sqrt{\tr(\Gamma)} -  \Lambda_{max}(\Gamma)~\eta_0 w(A)  - \tau~,
%\eeq
%where $k_0,\eta_0, \eta_1, \eta_2$ are constants which depend on the sub-Gaussian norm $\vertiii{ x_{ij} }_{\psi_2} = k$.
%\label{thm:corrSubG}
%\end{theo}

